Generating Graph-Like Logical Rules for Knowledge Graph Reasoning via Diffusion Models

Logical rules constitute a cornerstone of knowledge graph (KG) reasoning, valued for their interpretability and ability to model relational patterns. However, existing rule mining methods predominantly focus on simple chain-like rules and therefore neglect the richer relational information encoded in graph-like structures, such as cycles and branches. This limitation is further exacerbated by computational bottlenecks caused by the combinatorial explosion of the search space, which is especially challenging for graph-like rules. Meanwhile, generative approaches such as diffusion models, despite their success in other domains, cannot be directly applied to rule mining because their training objectives are not aligned with the goal of learning high-quality rules, and non-differentiable KG rule quality metrics cannot directly guide model optimization. To address these limitations, we propose GRiD, a framework that reformulates graph-like rule discovery as a discrete generative process conditioned on the target relation. GRiD employs a two-phase training strategy. First, supervised pre-training enables GRiD to capture structural priors from subgraphs sampled from the KG meta-graph. Subsequently, reinforcement learning is applied to fine-tune GRiD through policy gradient optimization guided directly by non-differentiable rule-quality metrics. Experiments on six benchmark datasets show that GRiD achieves competitive performance on KG completion tasks. Ablation studies confirm the efficiency and robustness of GRiD and further show that graph-like rules complement chain-like rules in KG completion. Our code and datasets are available in https://github.com/Haoxiang-Cheng/GRiD.

==> Tabs/tab_dataset.tex <==
% \begin{table}[h!]
%     \centering
%        \caption{Statistics of KGC datasets}
%        \label{table_dataset}
%        \renewcommand\arraystretch{1.2}
%         \begin{tabular}{cccc}
%     \toprule[1pt]
%         Dataset &\#Entity  &\#Relation &\#Facts\\
%      \hline
%       Family & 3,007 & 12 & 28,356 \\
% Kinship & 104 & 25 & 9,587 \\
% UMLS & 135 & 46 & 5,960 \\
% WN-18RR & 40,943 & 11 & 93,003 \\
% FB15K-237 & 14,541 & 237 & 310,116 \\
% YAGO3-10 & 123,182 & 37 & 1,089,040 \\

%        \bottomrule[1pt]
%    \end{tabular}
% \end{table}

\begin{table}[t]
    \centering
       \caption{Statistics of KGC datasets}
       \label{table_dataset}
        \resizebox{\linewidth}{!}{  
        \begin{tabular}{ccccccc}
    \toprule[1pt]
        Dataset & Family & Kinship & UMLS & WN-18RR & FB15K-237 & YAGO3-10 \\
     \hline
        \#Entity & 3,007 & 104 & 135 & 40,943 & 14,541 & 123,182 \\
        \#Relation & 12 & 25 & 46 & 11 & 237 & 37 \\
        \#Facts & 28,356 & 9,587 & 5,960 & 93,003 & 310,116 & 1,089,040 \\
       \bottomrule[1pt]
   \end{tabular}}
\end{table}


==> Tabs/tab_hyper.tex <==
\begin{table*}[t]
\centering
\caption{Experiment Settings}
\label{tab:hyperparameters}
\begin{tabular}{p{2.2cm}p{3cm}p{2cm}p{7cm}}
\toprule
\textbf{Category} & \textbf{Parameter} & \textbf{Default Value} & \textbf{Description} \\
\midrule
\multirow{3}{*}{\textbf{Graph Sampling}} 
 & Maximum length & 3 & Maximum path length for sampling chain-like rules \\
 & Anchor number & 500 & Number of anchor points per relation for sampling \\
 & Random seed & 3407 & Seed for reproducible sampling \\
\midrule

\multirow{4}{*}{\textbf{Diffusion}}
 & Time steps & 500 & Total number of diffusion timesteps \\
 & Cosine offset & 0.008 & Cosine scheduler offset for $\beta_t$ curve smoothness \\
 & Beta scale & 1.0 & Scaling factor for $\beta_t$ (clipped to [0.3, 1.5]) \\
 & Beta range & [$1\times10^{-5}$, 0.3] & Clipping range for $\beta_t$ values \\
\midrule
\multirow{3}{*}{\textbf{Optimization}}
 & Learning rate & $1\times10^{-3}$ & Adam learning rate for backbone network \\
 & Gradient clip & 5.0 & Gradient norm clipping value \\
 & Batch size & 32 & Batch size for supervised training \\
\midrule
\multirow{1}{*}{\textbf{Loss Function}}
 & Loss weights & [1.0, 0.2] & Weight ratio for perturbed versus retained positions \\
\midrule
\multirow{8}{*}{\textbf{Architecture}}
 & Time dimension & 64 & Time embedding dimension \\
 & Relation dimension & 64 & Relation embedding dimension \\
 & Condition dimension & 64/128 & Condition embedding dimension \\
 & Node dimension & 128 & Node embedding dimension \\
 & forward dimension & 256 & Feed-forward network dimension \\
 & Number of layers & 3 & Number of Graph Transformer layers \\
 & Number of heads & 4 & Number of attention heads \\
 & Dropout rate & 0.1 & Dropout rate \\
\midrule
\multirow{1}{*}{\textbf{Evaluation}}
 & Prediction number & 50 & Evaluation trigger for adaptive scheduling \\
\midrule
\multirow{5}{*}{\textbf{RL}}
 & RL iterations & 100 & Number of major RL iterations  \\
 & Entropy coefficient & $1\times10^{-3}$ & Entropy regularization coefficient for REINFORCE \\
 & EMA beta & 0.9 & Exponential moving average coefficient for baseline \\
 & Supervised epochs & 10 & Supervised epochs before RL training \\
 & Evaluation frequency & 2 & Evaluation interval during supervised pre-training \\
\bottomrule
\end{tabular}
\end{table*}


==> Tabs/tab_test.tex <==
\begin{table*}[t]
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}


==> Tabs/table_chain-rules.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.1}
\centering
\caption{Top chain-like rules learned by \model~on YAGO3-10.}
\resizebox{0.8\linewidth}{!}{%x
\begin{tabular}{c}
 \toprule[1pt]

 isLocatedIn$(x,y) \leftarrow $hasNeighbor$(x,z) \wedge $isLocatedIn$(z,y)$
  \\
  isLocatedIn$(x,y) \leftarrow $hasNeighbor$(x,z_1) \wedge $ dealsWith$(z_1,z_2) \wedge $ isLocatedIn$(z_2,y)$
  \\
  isLocatedIn$(x,y) \leftarrow $hasCapital$(x,z) \wedge  $participatedIn$(x,z)\wedge $happenedIn$(z,y)$\\

\hline


 isCitizenOf$(x,y) \leftarrow $LivesIn$(x,y)$  \\
 isCitizenOf$(x,y) \leftarrow $isMarriedTo$(x,z) \wedge $isCitizenOf$(z,y)$
\\
  isCitizenOf$(x,y) \leftarrow $hasAcademicAdvisor$(x,z_1) \wedge $ worksAt$(z_1,z_2) \wedge $ isLocatedIn$(z_2,y)$
\\ 

 
 \hline
 
 livesIn$(x,y) \leftarrow $worksAt$(x,z) \wedge $isLocatedIn$(z,y)$
\\
 livesIn$(x,y) \leftarrow $wasBornIn$(x,z) \wedge $isLocatedIn$(z,y)$
\\
livesIn$(x,y) \leftarrow $hasChild$(x,z_1) \wedge $ isMarriedTo$(z_1,z_2) \wedge $ livesIn$(z_2,y)$
\\ \hline
GraduatedFrom$(x,y) \leftarrow  $worksAt$(x,y)$
\\
 GraduatedFrom$(x,y) \leftarrow $hasAcademicAdvisor$(x,z) \wedge $worksAt$(z,y)$
\\ 
GraduatedFrom$(x,y) \leftarrow $hasAcademicAdvisor$(x,z_1) \wedge $ influences$(z_1,z_2) \wedge $ graduatedFrom$(z_2,y)$
\\
\hline
wasBornIn$(x,y) \leftarrow $hasChild$(z,x) \wedge $livesIn$(z,y)$ \\

wasBornIn$(x,y) \leftarrow $isMarriedTo$(x,z) \wedge $wasBornIn$(z,y) \wedge $isLocatedIn$(z,y)$ \\

wasBornIn$(x,y) \leftarrow $hasAcademicAdvisor$(x,z_1) \wedge $worksAt$(z_1,z_2) \wedge $isLocatedIn$(z_2,y)$
\\
\bottomrule[1pt]
\end{tabular}
}
\label{table_chain-rule}
% \vspace{-20pt}
\end{table*}


==> Tabs/table_graph-rules.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.1}
\centering
\caption{Top graph-like rules learned by \model~on YAGO3-10.}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c}

\toprule[1pt]
isLocatedIn$(x,y) \leftarrow $hasCapital$(x,z_1) \wedge $hasCapital$(y,z_1) \wedge $hasOfficialLanguage$(x,z_2) \wedge $hasOfficialLanguage$(y,z_2)$\\

isLocatedIn$(x,y) \leftarrow $exports$(x,z_1) \wedge $imports$(y,z_1) \wedge $hasCurrency$(x,z_2) \wedge $hasCurrency$(y,z_2)$\\

isLocatedIn$(x,y) \leftarrow $hasNeighbor$(x,z_1) \wedge $hasNeighbor$(y,z_1) \wedge $exports$(x,z_2) \wedge $imports$(y,z_2)$\\

\hline
 isCitizenOf$(x,y) \leftarrow $LivesIn$(x,y)$ $\wedge$  WorksAt$(x,y)$)  \\
 isCitizenOf$(x,y) \leftarrow $isMarriedTo$(x,z_1) \wedge$ isCitizenOf$(z_1,z_2) \wedge $Dealswith$(z_1,y)$
\\

isCitizenOf$(x,y) \leftarrow $GraduatedFrom$(x,z_1) \wedge $isLocatedIn$(z_1,y) \wedge $hasAcademicAdvisor$(x,z_2) \wedge $livesIn$(z_2,y)$

\\ 

 \hline
 
livesIn$(x,y) \leftarrow $worksAt$(x,z_1) \wedge $isLocatedIn$(z_1,y) \wedge $owns$(x,z_2) \wedge $isLocatedIn$(z_2,y)$\\

livesIn$(x,y) \leftarrow $isCitizenOf$(x,y) \wedge $hasChild$(x,z_1) \wedge $GraduatedFromAt$(z_1,z_2) \wedge $isLocatedIn$(z_2,y)$\\

livesIn$(x,y) \leftarrow $isMarriedTo$(x,z_1) \wedge $livesIn$(z_1,y) \wedge $worksAt$(x,z_2) \wedge $isLocatedIn$(z_2,y)$
\\ \hline
GraduatedFrom$(x,y) \leftarrow $isAffiliatedTo$(x,y) \wedge $created$(x,z_1) \wedge $isLocatedIn$(z_1,y)$ \\

GraduatedFrom$(x,y) \leftarrow $hasAcademicAdvisor$(x,z_1) \wedge $GraduatedFrom$(z_1,y) \wedge $worksAt$(x,y)$\\

GraduatedFrom$(x,y) \leftarrow $isMarriedTo$(x,z_1) \wedge $GraduatedFrom$(z_1,y) \wedge $isLocatedIn$(z_1,y)$
\\ \hline
wasBornIn$(x,y) \leftarrow $hasChild$(z_1,x) \wedge $wasBornIn$(z_1,y) \wedge $isLocatedIn$(z_1,y)$\\

wasBornIn$(x,y) \leftarrow $GraduatedFrom$(x,z_1) \wedge $WorksAt$(x,z_1) \wedge $LocatedIn$(z_1,y) \\

wasBornIn$(x,y) \leftarrow $GraduatedFrom$(x,z_1) \wedge $isLocatedIn$(z_1,y) \wedge $hasAcademicAdvisor$(x,z_2) \wedge $wasBornIn$(z_2,y)$\\

\bottomrule[1pt]
\end{tabular}
}
\label{table_graph-rule}
% \vspace{-20pt}
\end{table*}

